SpecMol: A Spectroscopy-Grounded Foundation Model for Multi-Task Molecular Learning

Large language models have emerged as transformative tools in molecular science, demonstrating remarkable potential in molecular property prediction and de novo molecular design. However, their application to spectroscopy remains notably limited, despite its foundational role in experimental molecular characterization and structural validation. Progress in spectroscopy-grounded reasoning has been hindered by the lack of standardized spectral representations and comprehensive evaluation protocols, making cross-study comparisons difficult. To bridge this gap, we present a unified framework for spectroscopy-grounded molecular modeling and evaluation. At its core, the SpecMol foundation model integrates spectral interpretation, molecular representation learning, and three-dimensional structure generation within a single interface. Complementing this, we establish SpecMol-Bench as a systematic evaluation protocol encompassing cross-modal tasks: spectra-to-structure elucidation, structure-to-spectra simulation, and SMILES-to-3D conformation generation. Under this unified framework, SpecMol achieves accurate spectra-driven structure elucidation and reproduces experimental nuclear magnetic resonance characteristics with high fidelity. The model also generates chemically valid three-dimensional conformations directly from SMILES strings and consistently outperforms existing general-purpose molecular language models across standardized evaluation metrics. Code is available at https://github.com/Eurekashen/SpecMol

==> files/experiment_setup.tex <==
\section{Experiments}
\subsection{Experimental Setup}

\noindent\textbf{Tasks and Data Split.}
We evaluate \textit{\mname} on a suite of downstream tasks spanning molecular question answering, symbolic translation between SMILES and IUPAC names, spectroscopy grounding between SMILES and spectra, and three-dimensional structure generation from SMILES or IUPAC strings. The task-wise training and testing distributions for supervised fine-tuning are summarized in Table~\ref{tab:sft_split}. For three-dimensional coordinate generation, we use a combined set comprising 8,329 training and 834 testing samples.
To prevent scaffold-level leakage in all structure-conditioned settings, we adopt a Bemis--Murcko scaffold split~\cite{bemis1996properties}.

% --- Table: SFT Data Split ---
\begin{table}[!htb]
\centering
\caption{Task-specific training and testing data distribution for supervised fine-tuning (SFT).}
\label{tab:sft_split}
\begin{tabular}{lcc}
\toprule
\textbf{Task} & \textbf{Train Samples} & \textbf{Test Samples} \\ \midrule
Molecule QA & 14,994 & 500 \\
SMILES to IUPAC & 13,727 & 100 \\
IUPAC to SMILES & 16,987 & 100 \\
SMILES to 3D Coord. & 8,329 & 834 \\
SMILES to Spec & 15,653 & 200 \\
Spec to SMILES & 12,000 & 200 \\ \bottomrule
\end{tabular}
\end{table}

\noindent\textbf{SpecMol-Bench.}
We curate \textbf{SpecMol-Bench} as a unified evaluation benchmark for spectroscopy-centered molecular tasks under consistent splits and protocols. SpecMol-Bench aggregates the supervised fine-tuning tasks shown in Table~\ref{tab:sft_split} into a standardized multi-task setting. This benchmark comprises 81,690 training instances and 1,834 test instances in total.\footnote{The benchmark aggregates multiple tasks; a single molecule may contribute instances to more than one task. Detailed construction and prompts are provided in the Supporting Information.}

\noindent\textbf{Pretraining Data.}
We continually pretrain \textit{\mname} with a large chemistry corpus and a multimodal molecular collection spanning molecular text, structures, and spectra. 
PubChem provides the primary source of molecular descriptions. 
To incorporate spectroscopy signals, we integrate experimental NMR from NMRBank~\cite{wang2025nmrextractor} and simulated spectra from QM9S, together with additional multimodal spectroscopic records from the Multimodal Spectroscopic Dataset~\cite{alberts2024unraveling}. 
The data composition is summarized in Table~\ref{tab:pretrain_data}. 
We apply standard quality control measures including the removal of salts and solvents, element and atom count constraints, deduplication by canonical SMILES, and the removal of any overlap with evaluation sets.
After filtering, we obtain $\sim$5M molecules and $\sim$0.2M spectrum--molecule pairs for pretraining.

% --- Table: Pretrain Data ---
\begin{table}[!htb]
\centering
\caption{Summary of pretraining data sources, spectrum classes, and types.}
\label{tab:pretrain_data}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lccccccc}
\toprule
\multirow{2}{*}{\textbf{Source}} & \multicolumn{4}{c}{\textbf{Spectrum Classes}} & \multicolumn{2}{c}{\textbf{Spectrum Type}} & \multirow{2}{*}{\textbf{Distribution}} \\ \cmidrule(lr){2-5} \cmidrule(lr){6-7}
 & \textbf{NMR} & \textbf{IR} & \textbf{MS} & \textbf{UV-Vis} & \textbf{Exp.} & \textbf{Sim.} & \\ \midrule
PubChem & / & / & / & / & / & / & 11,900,000 \\
QM9S & $\times$ & \checkmark & \checkmark & \checkmark & $\times$ & \checkmark & $\sim$130,000 \\
NMRBank & \checkmark & $\times$ & $\times$ & $\times$ & \checkmark & $\times$ & 225,809 \\
MultiModal & \checkmark & \checkmark & \checkmark & $\times$ & $\times$ & \checkmark & 790,000 \\ \bottomrule
\end{tabular}
\end{table}

\noindent\textbf{Baselines.}
We compare \textit{\mname} against three categories of baselines.
(1) \textbf{Generalist LLMs}: DeepSeek-V3~\cite{deepseekai2024deepseekv3technicalreport}, Qwen3-235B~\cite{qwen2025qwen25technicalreport}, Kimi-K2~\cite{kimiteam2025kimik2openagentic}, OpenAI o3~\cite{openai2025o3}, Gemini-2.5-Flash~\cite{geminiteam2025flash}, and GPT-5~\cite{openai2025gpt5}. 
(2) \textbf{Chemistry-specialist models}: \textit{ChemDFM-v2.0-14B}~\cite{zhao2025chemdfm} and \textit{InternS1-235B}~\cite{bai2025intern}. 
(3) \textbf{Task-specific tools}: STOUT~\cite{rajan2021stout} and OPSIN~\cite{lowe2022opsin} for SMILES$\leftrightarrow$IUPAC conversion.
For forward NMR simulation, we additionally report MestReNova~\cite{willcott2009mestre} where applicable.

\noindent\textbf{Implementation Details.}
\textit{\mname} is initialized from the \textbf{Qwen2.5-7B}~\cite{qwen2025qwen25technicalreport} base model. 
For all LLM baselines, we use a unified prompt template per task and fixed decoding parameters for reproducibility (temperature $=0$, top-$p=1$; max generation length and stop sequences are task-specific but identical across models). 
All outputs are post-processed with the same parser. Invalid or non-parsable generations (e.g., malformed tags or invalid SMILES) are counted as incorrect for exact-match metrics. 
For SMILES generation, we apply RDKit canonicalization before exact-match scoring and additionally report InChIKey-based accuracy. Full decoding and post-processing settings are provided in the Supporting Information.


\subsection{Evaluation Metrics}
\label{sec:evaluation}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/SpecMol-Bench.pdf}
    \caption{ SpecMol-Bench: A unified, chemistry-aware evaluation framework. Unlike traditional fragmented protocols, SpecMol-Bench evaluates performance using standardized metrics along three axes: symbolic correctness (strings), spectral fidelity (spectra), and physical plausibility (3D structures).}
    \label{fig:SpecMol_Bench}
\end{figure}

We evaluate performance along three axes: \textbf{(i) symbolic correctness} for molecular strings, \textbf{(ii) spectral fidelity} for spectrum generation, and \textbf{(iii) physical plausibility} for 3D structures (Figure~\ref{fig:SpecMol_Bench}). 
Below we summarize the metrics; complete definitions and implementation details are provided in the Supporting Information. Standardized preprocessing is applied to all models identically

\paragraph{Multiple-Choice Accuracy.}
For molecule QA, we report multiple-choice accuracy to determine whether the predicted option matches the ground-truth label.

\paragraph{Token and Sequence level Accuracy.}
For sequence generation tasks such as SMILES-IUPAC conversion, \textit{token accuracy} measures the fraction of correctly predicted tokens and \textit{sequence accuracy} measures exact-string matches. We additionally report an InChIKey-based accuracy by converting predicted and reference molecules to InChIKeys. A prediction is counted as correct if the InChIKeys match, which provides a representation-invariant measure for SMILES equivalence.

\paragraph{3D Structure Validity and Geometry.}
For 3D coordinate generation, we report:
(i) \textit{SDF Validity}, the percentage of parsable molecules;
(ii) \textit{Atom Clash}, the average number of severe steric overlaps;
(iii) \textit{Bond Violation}, the average number of abnormal bond lengths; and
(iv) \textit{Fingerprint Similarity}, computed as Tanimoto similarity over RDKit fingerprints (path-based, topological torsion, and atom-pair) between predicted and reference structures.

\paragraph{NMR Spectrum Assessment.}
For discrete NMR peak sets, we adopt a tolerance-based peak matching protocol.
For $^{13}$C NMR, we perform greedy one-to-one matching between predicted and ground-truth shifts within a tolerance of 0.5 ppm. We report precision (P), recall (R), F1 score, and mean absolute error over matched pairs. For $^{1}$H NMR, we match peaks within a tolerance of 0.12 ppm and report a weighted Jaccard similarity that jointly reflects shift accuracy and integration fidelity. Weights are defined by a Gaussian decay of the shift difference and scaled by the minimum proton count of the matched pair. We also benchmark unweighted set metrics and the vector cosine similarity score used in NMR-Solver~\cite{jin2025nmr}.

\paragraph{IR and MS Spectrum Assessment.}
For infrared and mass spectrometry spectra treated as continuous intensity distributions, we discretize spectra into vectors via binning at a resolution of 1~cm$^{-1}$ for IR and 1~m/z for MS. We report cosine similarity between predicted and ground-truth vectors to measure global spectral-shape and relative-intensity alignment.

\medskip
\noindent Together, these modality-specific protocols provide standardized and chemistry-aware assessment across spectra, strings, and 3D structures.

